A Multi-Agent Model for Polarization under Confirmation Bias in Social Networks

We describe a model for polarization in multi-agent systems based on Esteban and Ray's standard measure of polarization from economics. Agents evolve by updating their beliefs (opinions) based on an underlying influence graph, as in the standard DeGroot model for social learning, but under a confirmation bias; i.e., a discounting of opinions of agents with dissimilar views. We show that even under this bias polarization eventually vanishes (converges to zero) if the influence graph is strongly-connected. If the influence graph is a regular symmetric circulation, we determine the unique belief value to which all agents converge. Our more insightful result establishes that, under some natural assumptions, if polarization does not eventually vanish then either there is a disconnected subgroup of agents, or some agent influences others more than she is influenced. We also show that polarization does not necessarily vanish in weakly-connected graphs under confirmation bias. We illustrate our model with a series of case studies and simulations, and show how it relates to the classic DeGroot model for social learning.

==> confirmation-bias.tex <==
The incorporation of confirmation bias into our model
allows for the uncovering of new, interesting phenomena.
Fig.~\ref{fig:comparing-update-functions} illustrates
the evolution of polarization, starting from a
tripolar belief configuration, 
in a \emph{faintly communicating} 
influence graph (schematically depicted in Fig.~\ref{fig:interaction-graphs-faint}) %\Ifunfaint$, 
representing  a social network divided into two groups that 
evolve mostly separately, with little communication between 
them.\footnote{More precisely:
    $\Ifunfaint{\agent{i}}{\agent{j}}{=}0.5$, if $\agent{i},\agent{j}$ are both
    ${\leq} \ceil{\nicefrac{n}{2}}$ or both ${>} \ceil{\nicefrac{n}{2}}$, 
    and $\Ifunfaint{\agent{i}}{\agent{j}}{=}0.1$ otherwise.} 
%\todo{Santiago: Bernardo, I re-ran the simulations but given that we changed our initial belief configurations, the old mildly polarized is similar to the new extremely. Shall we change to those or keep it with the new mildly polarized configuration? }
If agents employ the original update (Fig.\ref{fig:comparing-classic-update}), they are quickly influenced towards a midpoint between their beliefs,
reaching consensus and eliminating polarization.
On the other hand, if agents employ confirmation-bias update
(Fig.\ref{fig:comparing-confirmation-bias}),
convergence happens significantly more slowly, extending
polarization further in time.
Note that, in this case, confirmation bias emphasizes the
non-monotonicity of polarization: since
each group reaches an internal consensus  relatively quickly,
polarization increases; but as each group slowly communicates,
general consensus is eventually achieved.
%\todo[disable]{Santiago, add the polarization lower part to these graphs.}



% As in the \emph{classical update}, it is of our interest to know if the opinions converge when using this update-function. 
Note that the confirmation-bias update function generalizes Def.\ref{def:rational-update-function}, since the latter
is the special case of the former in which the confirmation-bias 
factor is always 1.
The proof of Th.\ref{theorem:scc-convergence} can
be easily modified (see Appendix~\ref{sec:proofs}) to show that, 
also under confirmation bias,
% ~\footnote{
% More precisely:
% \begin{enumerate}
%     \item If for a particular time $t$: $\forall \agent{i}, \agent{j} \in \Agents, \CBfun{i}{j}{t} > 0$ (when $\forall \agent{i} \in \Agents, \Bfun{i}{t} \notin \{0,1\}$) the proof follows the same steps as the proof on Theorem \ref{theorem:scc-convergence}, but with a looser $\epsilon$, since it will also be multiplied by $\CBfunM{t} = \underset{\agent{i},\agent{j} \in \Agents}{\min} \CBfun{i}{j}{t}$. 
%     \item Else if no agents have belief equal to $0$ or $1$, all beliefs do not change throughout time, since the \emph{confirmation-bias factor} is so big that no agent is influenced by agents with different belief.
%     \item Else some agent has belief different from $0$ and $1$, and we can show that after $|\Agents|-1$ time steps we fall on case $1$.
% \end{enumerate}
% }
in strongly connected influence graphs all agents' beliefs eventually converge to the same value (with the sole exception of a society in which all agents possess extreme beliefs of 0 or 1).
This implies that polarization vanishes over time, even if at a slower pace, in the absence of external influences.
This is formalized below.

\begin{theorem}[Partial belief consensus under confirmation bias]\label{theorem:scc-convergence-confirmation-bias} 
In a strongly connected influence graph and under the confirmation-bias update-function, if there exists an agent $\agent{k} \in \Agents$ such that $\Bfun{k}{0} \notin \{0,1\}$ then for every $\agent{i}, \agent{j} \in \Agents$, $\lim_{t \to \infty} \Bfun{i}{t} = \lim_{t \to \infty} \Bfun{j}{t}$. Otherwise for every $\agent{i} \in \Agents$, $\Bfun{i}{t} = \Bfun{i}{t+1} \in \{0,1\}$.
\end{theorem}

% However, the technique used in the more general Theorem~\ref{} 
% \todo{M\'ario: Add here the reference to the theorem of general case} cannot be applied to confirmation-bias update (since the
% Markov update matrix would not be constant over time), 
% and the problem of whether polarization always converges in 
% weakly connected graphs in  he presence of this kind of bias 
% is still open. 
% We leave it as future work.
